InvestESG: A multi-agent reinforcement learning benchmark for studying climate investment as a social dilemma

InvestESG is a novel multi-agent reinforcement learning (MARL) benchmark designed to study the impact of Environmental, Social, and Governance (ESG) disclosure mandates on corporate climate investments. The benchmark models an intertemporal social dilemma where companies balance short-term profit losses from climate mitigation efforts and long-term benefits from reducing climate risk, while ESG-conscious investors attempt to influence corporate behavior through their investment decisions. Companies allocate capital across mitigation, greenwashing, and resilience, with varying strategies influencing climate outcomes and investor preferences. We are releasing open-source versions of InvestESG in both PyTorch and JAX, which enable scalable and hardware-accelerated simulations for investigating competing incentives in mitigate climate change. Our experiments show that without ESG-conscious investors with sufficient capital, corporate mitigation efforts remain limited under the disclosure mandate. However, when a critical mass of investors prioritizes ESG, corporate cooperation increases, which in turn reduces climate risks and enhances long-term financial stability. Additionally, providing more information about global climate risks encourages companies to invest more in mitigation, even without investor involvement. Our findings align with empirical research using real-world data, highlighting MARL's potential to inform policy by providing insights into large-scale socio-economic challenges through efficient testing of alternative policy and market designs.

==> 3-Method.tex <==
\section{Problem Setting}
Corporations face two key trade-offs in climate action. The first is between short-term costs and long-term benefits, as climate efforts often require upfront investments with returns realized over time. The second is between self-interest and collective benefit, as emission reductions benefit all, but the costs are borne by those who act, which incentivizes free-riding and undermines collective action. These trade-offs  motivate us to conceptualize corporate climate actions as an intertemporal social dilemma \citep{leibo2017multi, bisaro2016governance}, which by definition, involves a conflict between immediate self-interest and longer-term collective interests. Given the magnitude and complexity of the global market, we develop a conceptual model to capture key trade-offs, drawing on well-established finance and economics literature that addresses similar questions. For instance, Pastor et al. (2021) and Pedersen et al. (2021) proposed analytical models of single-period equilibria, where companies either choose or are assigned fixed levels of "greenness," and investors optimize portfolios to balance financial returns with preferences for green assets. We follow a similar setting where companies choose mitigation effort levels every period and receive a single metric ESG score that reflects their greenness. Investors derive utility from the profits generated by their portfolios and investing in firms with high ESG scores depending on investors' ESG preference, which we call "ESG-consciousness". We extend these frameworks by (1) modeling the evolution of firm-investor strategies over the long run, which poses significant analytical and numerical challenges \citep{pakes2001stochastic}, (2) incorporating climate evolution, where risks worsen over time but can be mitigated by firm efforts, and (3) introducing greenwashing \citep{lyon2011greenwash} where companies cheaply inflate ESG scores without genuine mitigation, which raises issues of information asymmetry and principal-agent problems \citep{grossman1992analysis}.

We aim to address the following research questions: (1) Do ESG-conscious investors incentivize companies to undertake mitigation efforts, and how does the level of ESG-consciousness influence these outcomes? (2) Does the presence of heterogeneous investors lead to bifurcation among agents, where only some companies engage in mitigation and attract investments from ESG-conscious investors, while others and their investors opt to free-ride? (3) Are companies likely to engage in greenwashing? (4) What measures can enhance the effectiveness of ESG disclosure mandates?

\section{The InvestESG Environment} \label{sec:environment}
InvestESG is a MARL benchmark environment designed to evaluate the impact of ESG disclosure mandates on corporate climate investments.
% We model the environment as an intertemporal social dilemma where company agents face short-term profit losses from climate mitigation efforts, but these actions reduce long-term climate risks, benefiting all. 
% \textcolor{red}{JZL: a minor quibble about language here, I would avoid saying ``X models a sequential social dilemma where...''. It sounds like a category error to me. The way I see it at least, a sequential social dilemma is a kind of model (or being an SSD is a property that a model may or may not have). So I would typically say something like ``Here we model phenomenon X using a sequential social dilemma''. In terms of philosophy of science jargon, I see the sequential social dilemma concept as explanans not explanandum.}
% \subsection{Environment Setup} 
The simulation starts in 2021 and runs through 2120, with each period $t$ corresponding to one year. The environment includes two main components: (1) an evolving climate and economic system, and (2) two types of agents: $M$ company agents $\mathcal{C}_i$ for $i \in \{1, \dots, M\}$ and $N$ investor agents $\mathcal{I}_j$ for $j \in \{1, \dots, N\}$.

\begin{wrapfigure}{R}{0.35\textwidth}
    \vspace{-0.5cm}
    \begin{subfigure}[t]{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth]{iclr2025/figures/status_quo.pdf}
        \caption{Environment dynamics over the course of a single 100 year episode.}
        \label{fig:env_dynamics}
    \end{subfigure}
    \begin{subfigure}[t]{0.35\textwidth}
    \centering
        \includegraphics[width=\textwidth]{iclr2025/figures/status_quo_climate_occurence.pdf}
        \captionsetup{width=\textwidth}
        \caption{Average number of severe climate event occurrences over 10-year period. }
        \label{fig:env_climate_event_occurrence}
    \end{subfigure}
    \caption{\footnotesize{Status quo scenario where all agents are only profit-motivated. In (a), mitigation spending (blue curve) is minimal, leading climate risk (yellow curve) to increase over time. Adverse weather event occurrences are shown as dotted lines; red lines indicate multiple adverse events in a single year. In (b), increasing climate risk leads to more frequent occurrence of severe climate events over time. }}
    \vspace{-0.2cm}
\end{wrapfigure}
\textbf{Climate and Economic Dynamics.}
The environment is characterized by three climate risk parameters: extreme heat probability ($P_t^h$), heavy precipitation probability ($P_t^p$), and drought probability ($P_t^d$) in year $t$. Initial climate risks are set to $P_0^h = 0.28$, $P_0^p = 0.13$, and $P_0^d = 0.17$ following the IPCC estimate \citep{IPCC2021}, resulting in an overall climate risk of $P_0 = 0.48$, the probability of at least one adverse climate event in a year. Without mitigation efforts, these risks increase linearly over time,  reaching the IPCC's \SI{4}{\degreeCelsius} scenario scenario by 2100, which corresponds to the 80th period in our 100-period simulation. By that point, we observe $\overline{P}_{80}^h = 0.94$, $\overline{P}_{80}^p = 0.27$, and $\overline{P}_{80}^d = 0.41$ (or an overall climate risk of $\overline{P}_{80} = 0.97$). We then extrapolate this trend through to period 100.
% which assumes high carbon emissions \citep{IPCC2021}. With no mitigation efforts, by 2100 these risks reach $\overline{P}_{80}^h = 0.94$, $\overline{P}_{80}^p = 0.27$, and $\overline{P}_{80}^d = 0.41$, yielding an overall climate risk of $\overline{P}_{80} = 0.97$.
Figure \ref{fig:env_dynamics} depicts how increased climate risks and adverse climate events increase over time in a  scenario where companies are solely profit-motivated. Company agents can mitigate the growth of climate risk by investing in emissions reduction. The change in climate risk $P_t^e$ for event $e \in \{h, p, d\}$ in year $t$ is governed by the function:
\begin{equation}
    P_{t}^e = \frac{\mu_e t}{1 + \lambda_e U_{t,m}} + P_0^e, \quad \text{for } e \in \{h, p, d\},
    \label{eq:climate_risk}
\end{equation}
%\(P_t^e = \frac{\mu_e t}{1 + \lambda_e U_{t,m}} + P_0^e\), 
where $U_{t,m}$ is the cumulative mitigation spending from all agents by period $t$. If $U_{t,m} = 0$, risks increase linearly to reach $\overline{P}_{80}^e$ by 2100 as explained earlier. When $U_{t,m} > 0$, the growth rate of climate risk decreases. The parameters $\lambda_e$ are calibrated based on \cite{IPCC2022}, which estimates that an annual mitigation investment of \$2.3 trillion is required to achieve IPCC's \SI{1.5}{\degreeCelsius} scenario. The model fits $\lambda_e$ so that such investment levels would yield \SI{1.5}{\degreeCelsius} scenario climate risks by 2100.
% For each type of climate events, parameters $\mu_e$ and $\lambda_e$ are calibrated based on IPCC's \SI{1.5}{\degreeCelsius} scenario. \cite{IPCC2022} estimates that \$2.3 trillion per year spending is needed to limit temperature to the \SI{1.5}{\degreeCelsius} scenario, which has an overall climate risk of about 0.60 by year 2100.
Climate events are modeled as independent Bernoulli processes, allowing for multiple events within a year (red dashed lines in Figure \ref{fig:env_dynamics}). Let \( X_{t,h}, X_{t,p}, X_{t,e} \in \{0,1\} \) represent the occurrence of each climate event, and \( X_t \) denote the total number of events in period \( t \), determined by Equation \ref{eq:climate_event}.
\begin{equation}
    X_t = X_{t,h} + X_{t,p} + X_{t,e}, \quad \text{where } X_{t,e} \sim \text{Bernoulli}(P_{t}^e), \quad \text{for } e \in \{h, p, d\}.
    \label{eq:climate_event}
\end{equation}
In addition to the evolving climate risks, the environment incorporates a baseline \textit{economic growth rate} $\gamma$, set to 10\% by default, aligned with the historical average annual return of the S\&P 500 over the past century \citep{Damodaran2024}. Company agents' capital levels $K_t^{\mathcal{C}_i}$ grow at rate $\gamma$ each year, barring climate events. If an adverse event occurs, company agents lose a portion of their total capital according to their respective \textit{climate resilience} parameter $L_t^{\mathcal{C}_i}$. If economic losses drive a company's remaining capital into negative territory, the company is declared bankrupt.

\textbf{Company Action Space.} Each company agent $\mathcal{C}_i$ in period $t$ selects actions from a continuous vector $\mathbf{u}_t^{\mathcal{C}_i} = (u_{t,m}^{\mathcal{C}_i}, u_{t,g}^{\mathcal{C}_i}, u_{t,r}^{\mathcal{C}_i})$, where $u_{t,m}^{\mathcal{C}_i}$ represents the share of capital allocated to mitigation, $u_{t,g}^{\mathcal{C}_i}$ to greenwashing, and $u_{t,r}^{\mathcal{C}_i}$ to building climate resilience. The action space for each company is defined as a continuous 3-dimensional unit cube, $\mathcal{U}_t^{\mathcal{C}_i} = [0, 1]^3$. If the sum of the three ratios exceeds 1 in any period, the company agent is deemed to be overspending, resulting in bankruptcy. Mitigation spending directly reduces the system-wide climate risk as explained above. Greenwashing involves deceptive marketing or accounting tactics that allow companies to appear climate-friendly at a low cost without providing any real benefits to society \citep{de2020concepts, yang2020greenwashing}. Resilience spending enhances the company's climate resilience by lowering its vulnerability $L_t^{\mathcal{C}_i}$, but it does not reduce emissions and therefore does not mitigate system-wide climate risk. In the default setting, we disable greenwashing and resilience spending to focus on testing companies' mitigation efforts. These options are later enabled to examine their effects, as will become clear in Section \ref{sec:results}.  

\textbf{Investor Action Space.} Investor agents first select the companies they want to invest in. Specifically, agent $\mathcal{I}_j$ in period $t$ selects an action from a binary vector of length $M$, $\mathbf{a}_t^{\mathcal{I}_j} = (a_{t,1}^{\mathcal{I}_j}, \dots, a_{t,M}^{\mathcal{I}_j})$, corresponding to the $M$ company agents. Each entry $a_{t,i}^{\mathcal{I}_j} = 1$ indicates that investor $\mathcal{I}_j$ invests in company $\mathcal{C}_i$ in period $t$, and $a_{t,i}^{\mathcal{I}_j} = 0$ otherwise. The investor's action space at time $t$ is thus $\mathcal{A}_t^{\mathcal{I}_j} = \{0, 1\}^M$. Once the choices are made, investors capitals are distributed equally among these chosen companies, as will be detailed later in Equation \ref{eq:interim_capital}.

\textbf{Modeling ESG Disclosure.} With the ESG disclosure mandate in place, each company agent receives an updated ESG score $Q_{t+1}^{\mathcal{C}_i}$ in period $t$, calculated as 
\begin{equation} \label{eq:esg_score}
    Q_{t+1}^{\mathcal{C}_i} = u_{t,m}^{\mathcal{C}_i} + \beta u_{t,g}^{\mathcal{C}_i}, 
\end{equation}
where $\beta > 1$ indicates that greenwashing is cheaper than genuine mitigation in terms of building an ESG-friendly image. This mirrors simple ESG ratings provided by some agencies, which typically range from 1 to 100 \citep{SPGlobalESGScores} or use letter-based ratings \citep{MSCIESGRatings}. 

\textbf{State and Observation Space.}
The environment simulates a partially observable Markov game $\mathcal{M}$ defined over a continuous, multi-dimensional state space. The system state at period $t$ is characterized by the three climate risk parameters $\mathbf{P}_t = (P_t^h, P_t^p, P_t^d)$, each company agent's state vector $\mathbf{S}_t^{\mathcal{C}_i} = (K_t^{\mathcal{C}_i}, Q_t^{\mathcal{C}_i}, L_t^{\mathcal{C}_i})$, where $K_t^{\mathcal{C}_i}$ is the capital level, $Q_t^{\mathcal{C}_i}$ is the ESG score, and $L_t^{\mathcal{C}_i}$ is the climate resilience. Each investor agent's state is represented by their investment portfolio and cash levels $\mathbf{S}_t^{\mathcal{I}_j} = (H_{t,1}^{\mathcal{I}_j}, \dots, H_{t,M}^{\mathcal{I}_j}, C_t^{\mathcal{I}_j})$, where $H_{t,i}^{\mathcal{I}_j}$ represents investor $\mathcal{I}_j$'s holdings in company $\mathcal{C}_i$, and $C_t^{\mathcal{I}_j}$ is the investor's cash level. The full system state at period $t$ is thus \(\mathcal{S}_t = \left( \mathbf{P}_t, \{ \mathbf{S}_t^{\mathcal{C}_i} \}_{i=1}^M, \{ \mathbf{S}_t^{\mathcal{I}_j} \}_{j=1}^N \right)\). All company and investor agents share a common observation space, denoted as $\mathcal{O}_t$. In the default setting, \(\mathcal{O}_t = \left(\{ \mathbf{S}_t^{\mathcal{C}_i} \}_{i=1}^M, \{ \mathbf{S}_t^{\mathcal{I}_j} \}_{j=1}^N \right)\). Extensions that incorporate additional observable information, like climate risk, are explored in Section \ref{sec:results}. 

\textbf{State Transition.} The environment's state transition $\mathcal{T}$ proceeds as follows. At the beginning of period $t$, investors collect their investment holdings from period $t-1$ and redistribute their capital according to $\mathbf{a}_t^{\mathcal{I}_j}$. Denote \( ||a_t||_1^{\mathcal{I}_j} = \sum_{i=1}^M a_{t,i}^{\mathcal{I}_j} \) as the number of companies investor \( \mathcal{I}_j \) invests in during period \( t \) and let \( K_t^{\mathcal{I}_j} = \sum_{i=1}^M H_{t,i}^{\mathcal{I}_j} + C_t^{\mathcal{I}_j} \) represent the total capital of investor \( \mathcal{I}_j \) at the start of period \( t \). Companies reach an interim capital level after returning old investments, $\sum_{j=1}^N H_{t,i}^{\mathcal{I}_j}$, and receiving new ones, with the investment from investor $\mathcal{I}_j$ calculated as $a_{t,i}^{\mathcal{I}_j} \frac{K_t^{\mathcal{I}_j}}{||a_t||_1^{\mathcal{I}_j}}$ or $0$ if the investor opts out of investing, as shown in Equation \ref{eq:interim_capital}.
\begin{equation}
    K_{t+1, interim}^{\mathcal{C}_i} = K_{t}^{\mathcal{C}_i} - \sum_{j=1}^N H_{t,i}^{\mathcal{I}_j} + 
    \sum_{j=1}^N 
    a_{t,i}^{\mathcal{I}_j} \frac{K_t^{\mathcal{I}_j}}{||a_t||_1^{\mathcal{I}_j}}
    % \begin{cases}
    %     a_{t,i}^{\mathcal{I}_j} \frac{K_t^{\mathcal{I}_j}}{||a_t||_1^{\mathcal{I}_j}}, & \text{if } ||a_t||_1^{\mathcal{I}_j} \neq 0 \\
    %     0, & \text{if } ||a_t||_1^{\mathcal{I}_j} = 0
    % \end{cases} 
    , 
    \quad \text{for } i = 1, \dots, M
    \label{eq:interim_capital}
\end{equation}
Companies then make climate-related spending using the interim capital, as described in Equations \ref{eq:total_mitigation} to \ref{eq:total_resilience}. Here, \( U_{t,m} \) represents the cumulative mitigation spending by all company agents up to period \( t \), while \( U_{t,r}^{\mathcal{C}_i} \) denotes the cumulative resilience spending by company \( \mathcal{C}_i \).
\begin{equation}
    U_{t,m} = U_{t-1,m} + \sum_{i=1}^M u_{t,m}^{\mathcal{C}_i} \times K_{t+1, interim}^{\mathcal{C}_i}
    \label{eq:total_mitigation}
\end{equation}
\begin{equation}
    U_{t,r}^{\mathcal{C}_i} = U_{t-1,r}^{\mathcal{C}_i} + u_{t,r}^{\mathcal{C}_i} \times K_{t+1, interim}^{\mathcal{C}_i} \quad \text{for } i = 1, \dots, M
    \label{eq:total_resilience}
\end{equation}
 While $U_{t,m}$ is then plugged into Equation \ref{eq:climate_risk} where system climate risks are updated. Equation \ref{eq:resilience} states that a company’s climate resilience, $L_t^{\mathcal{C}_i}$, scales with the proportion of cumulative resilience investment relative to its capital, and that increasing resilience becomes progressively more challenging due to diminishing returns \citep{IPCC2022WG2}.
\begin{equation}
    L_t^{\mathcal{C}_i} = L_0^{\mathcal{C}_i} \exp{(-\eta^{\mathcal{C}_i} \frac{U_{t-1,r}^{\mathcal{C}_i}+u_{t,r}^{\mathcal{C}_i}K_{t+1, interim}^{\mathcal{C}_i}}{K_{t+1, interim}^{\mathcal{C}_i}})}, \quad \text{for } i = 1, \dots, M .\label{eq:resilience}
\end{equation}
At the same time, the occurrence of climate events are simulated according to Equation \ref{eq:climate_event}, and companies receive updated ESG scores based on Equation \ref{eq:esg_score}. Afterwards, companies' profit margins, $\rho_t^{\mathcal{C}_i}$, are computed using Equation \ref{eq:profit_margin}, factoring in climate-related spendings $u_{t,m}^{\mathcal{C}_i}$, $u_{t,g}^{\mathcal{C}_i}$, $u_{t,r}^{\mathcal{C}_i}$, default economic growth $\gamma$, and losses due to climate events, which are influenced by companies' climate vulnerability $L_t^{\mathcal{C}_i}$ and the number of climate events $X_t$ as defined in Equation \ref{eq:climate_event}:
\begin{equation}
    \rho_t^{\mathcal{C}_i} = (1 - u_{t,m}^{\mathcal{C}_i} - u_{t,g}^{\mathcal{C}_i} - u_{t,r}^{\mathcal{C}_i}) (1+\gamma) (1 - X_t L_t^{\mathcal{C}_i}) - 1, \quad \text{for } i = 1, \dots, M.
    \label{eq:profit_margin}
\end{equation}
Company capitals $K_{t+1}^{\mathcal{C}_i}$, investor holdings $H_{t+1,i}^{\mathcal{I}_j}$, and investor cash positions $C_{t+1}^{\mathcal{I}_j}$ are updated according to Equations \ref{eq:capital_update} to \ref{eq:cash_flow}.  Company capitals $K_{t+1}^{\mathcal{C}_i}$ are updated according to Equation \ref{eq:capital_update} by scaling the interim capital levels by profit margin. 
\begin{equation}
    K_{t+1}^{\mathcal{C}_i} = (1+\rho_t^{\mathcal{C}_i}) K_{t+1, interim}^{\mathcal{C}_i}, \quad \text{for } i = 1, \dots, M.
    \label{eq:capital_update}
\end{equation}
Equation \ref{eq:investment} adjusts investor holdings based on company profit margins in their portfolios. 
\begin{equation}
    H_{t+1,i}^{\mathcal{I}_j} = a_{t,i}^{\mathcal{I}_j}(1 + \rho_t^{\mathcal{C}_i}) \frac{K_t^{\mathcal{I}_j}}{||a_t||_1^{\mathcal{I}_j}}, \quad \text{for } i = 1, \dots, M, j = 1, \dots, N.
    % H_{t+1,i}^{\mathcal{I}_j} = \begin{cases}
    %     a_{t,i}^{\mathcal{I}_j}(1 + \rho_t^{\mathcal{C}_i}) \frac{K_t^{\mathcal{I}_j}}{||a_t||_1^{\mathcal{I}_j}}, & \text{if } ||a_t||_1^{\mathcal{I}_j} \neq 0 \\
    %     0, & \text{if } ||a_t||_1^{\mathcal{I}_j} = 0
    % \end{cases}, \quad \text{for } i = 1, \dots, M, j = 1, \dots, N.
    \label{eq:investment}
\end{equation}
If an investor chooses not to invest, all capital remains as cash, as shown in Equation \ref{eq:cash_flow}
\begin{equation}
    C_{t+1}^{\mathcal{I}_j} = \begin{cases}
         0, & \text{if } ||a_t||_1^{\mathcal{I}_j} \neq 0 \\
         K_t^{\mathcal{I}_j}, & \text{if } ||a_t||_1^{\mathcal{I}_j} = 0
     \end{cases}, \quad \text{for } j = 1, \dots, N. \label{eq:cash_flow}
\end{equation}
\textbf{Rewards.} The single-period reward for company \( \mathcal{C}_i \) is solely based on its profit margin, given by \( r_t^{\mathcal{C}_i} = K_{t+1}^{\mathcal{C}_i} - K_{t+1, interim}^{\mathcal{C}_i} \) for \( i = 1, \dots, M \), reflecting the assumption that companies are profit-driven.  The reward for investor \( \mathcal{I}_j \) is \(r_t^{\mathcal{I}_j} = \frac{K_{t+1}^{\mathcal{I}_j} - K_t^{\mathcal{I}_j}}{K_t^{\mathcal{I}_j}} + \alpha^{\mathcal{I}_j} \frac{\sum_{i=1}^M H_{t+1,i}^{\mathcal{I}_j} Q_{t+1}^{\mathcal{C}_i}}{\sum_{i=1}^M K_{t+1}^{\mathcal{I}_j}}\) for \( j = 1, \dots, N \). The first component is the portfolio return ratio, and the second component represents the weighted average ESG score of the investor’s portfolio adjusted by the investor’s ESG preference, \( \alpha^{\mathcal{I}_j} \).


